Autoregressive Density Modeling with the Gaussian Process Mixture Transition Distribution

We develop a mixture model for transition density approximation, together with soft model selection, in the presence of noisy and heterogeneous nonlinear dynamics. Our model builds on the Gaussian mixture transition distribution (MTD) model for continuous state spaces, extending component means with nonlinear functions that are modeled using Gaussian process (GP) priors. The resulting model flexibly captures nonlinear and heterogeneous lag dependence when several mixture components are active, identifies low-order nonlinear dependence while inferring relevant lags when few components are active, and averages over multiple and competing single-lag models to quantify/propagate uncertainty. Sparsity-inducing priors on the mixture weights aid in selecting a subset of active lags. The hierarchical model specification follows conventions for both GP regression and MTD models, admitting a convenient Gibbs sampling scheme for posterior inference. We demonstrate properties of the proposed model with two simulated and two real time series, emphasizing approximation of lag-dependent transition densities and model selection. In most cases, the model decisively recovers important features. The proposed model provides a simple, yet flexible framework that preserves useful and distinguishing characteristics of the MTD model class.

==> sec_extensions.tex <==
% \section{Extensions}
% \label{sec:extensions} 

% In this section, we motivate and propose two extensions of the GPMTD model. The first relaxes Gaussianity of each mixture component and the second relaxes additivity to allow higher-order interactions necessary for an important application of the GPMTD. We provide details for implementation and discussion.


\section{Higher-order interactions with the GPMMTD}
\label{sec:gpmmtd}

In this section, we motivate and propose an extension of the GPMTD model that relaxes additivity to allow higher-order interactions necessary for some GPMTD model applications. This need was identified with the time-delay embedding example in Sec \ref{sec:appdata2d}. Here, we provide details for the extension, including implementation and discussion. Details for a second possible extension relaxing Gaussianity of each mixture component are presented in Appendix \ref{sec:appendix_skew}.

Allowing smooth nonlinear functions to the mixture means adds significant flexibility beyond the models in \citet{le1996gmtd}. However, using single-lag dependence in each mixture component of (\ref{eq:gpmtd1}) limits the scope of the GPMTD primarily to heterogeneous mixture error distributions and/or selection of a single relevant lag. To accurately model high-order transition surfaces with low noise in the GPMTD framework, it becomes necessary to admit $f$ functions of multiple lags. Although the transition mean resulting from the standard GPMTD model is additive and can approximate functions with mild interactions of inputs, the mixture of densities (rather than means) can result in the transition mean function falling in a region of low density, as seen in the time-delay embedding example of Section \ref{sec:appdata2d}. 

The most common approach to modeling functions with several inputs in the Gaussian process regression framework involves separable covariance functions, composed through the product of single-variable correlation functions \citep{rasmussen2006gp}. %This covariance structure naturally arises when one considers the process resulting from the product of independent functions, each modeled with an independent GP. 
Product correlation functions allow the length scale parameter to induce variable selection in automatic relevance determination (ARD, \citealp{neal1996ARD}). We present an alternative to ARD in the context of lag selection with an extension of the GPMTD model that follows the mixture of mixture transition distribution construction of \citet{heiner2019MMTDarXiv}. For positive integer $R < L$, the general model is given by
\begin{align}
\label{eq:GPMMTDtrans}
F_t(y_t & \mid y_{t-1}, \ldots, y_1) = \Lambda_0 \Ndist\left( y_t \mid \mu_0, \sigma_0^2 \right) + \nonumber \\
& \Lambda_1 \sum_{\ell=1}^L \lambda_{\ell}^{(1)} \Ndist \left( y_t \mid \mu_\ell + f_\ell^{(1)}(y_{t-\ell}), \sigma_{1,\ell}^2 \right) +  \\
& \Lambda_2 \underset{1 \le \ell_1 < \ell_2 \le L}{\sum \sum} \lambda_{(\ell_1, \ell_2)}^{(2)} \Ndist \left( y_t \mid \mu_{\ell_1, \ell_2}^{(2)} + f_{\ell_1, \ell_2}^{(2)}(y_{t-\ell_1}, y_{t-\ell_2}), \sigma_{2,\ell_1, \ell_2}^2 \right) \, + \ldots + \nonumber \\
& \Lambda_R \underset{1 \le \ell_1 < \ldots < \ell_R \le L}{\sum \ldots \sum} \lambda_{(\ell_1, \ldots, \ell_R)}^{(R)} \Ndist \left( y_t \mid \mu_{\ell_1, \ldots, \ell_R}^{(R)} + f_{\ell_1, \ldots, \ell_R}^{(R)}(y_{t-\ell_1}, \ldots, y_{t-\ell_R}), \sigma_{R,\ell_1, \ldots, \ell_R}^2 \right) \nonumber \, ,
\end{align}
with $\lambda^{(r)}_{(\ell_1, \ldots, \ell_r)} \in \bm{\lambda}^{(r)}$, a probability vector of length ${L \choose r}$, for $r = 1, \ldots, R$. We propose to simplify (\ref{eq:GPMMTDtrans}) by specifying only one set of parameters $(\mu, f, \sigma^2)$ for all mixture components at a given level $r > 1$, in conjunction with a sparse prior for each $\{\bm{\lambda}^{(r)} : r=2,\ldots,R \}$ that favors selection of only one component. One possibility is the sparse Dirichlet mixture (SDM) prior, also introduced in \citet{heiner2019spv}. Retaining the SBM prior on $\bm{\Lambda} = (\Lambda_0, \Lambda_1, \ldots, \Lambda_R)$ and $\bm{\lambda}^{(1)}$ preserves characteristics of the original GPMTD model and encourages shrinkage of the new, over-specified model. We will refer to the simplified specification as the canonical Gaussian process mixture of mixture transition distributions (GPMMTD) model.

%% covariance function spec.
The model in (\ref{eq:GPMMTDtrans}) can be flattened to a GPMTD representation with higher-order functions $\{f\}$. Increasing the number of arguments to each $f$ represents the primary innovation and challenge of the GPMMTD model. If we select $R$ to be modest and significantly below the lag horizon $L$, we can specify more general covariance functions than the standard isotropic or separable ARD kernels. One option relaxes isotropy (but retains stationarity) by replacing the Euclidean distance input of the squared exponential or Mat\'ern correlation function with a Mahalanobis distance $d = \sqrt{ (\bm{x} - \bm{x}')^\top \bm{\Psi} (\bm{x} - \bm{x}') }$ for positive-definite matrix $\bm{\Psi}$ (as in \citealp{ecker1999anisotropy}). That the parameters in $\bm{\Psi}$ are not identifiable and grow quadratically with the dimension of $\bm{x}$ can be addressed with informative priors and maintaining a moderate value of $R$.

The hierarchical formulation of the GPMMTD again utilizes augmentation with latent variables $Z_t \in \{0,1,\ldots,R\}$ and $\bm{z_t} \in \cup_{r} \{ (\ell_1, \ldots, \ell_r) : 1 \le \ell_1 < \ldots < \ell_r \le L \}$, and is given as follows. For $t = L+1, \ldots, T$; $\ell = 1, \ldots, L$, $1 \le \ell_1 < \ldots < \ell_r \le L$; and $r=0,1, \ldots, R$, we have
\begin{align}
\label{eq:GPMMTDhier}
    y_t \mid %\bm{x}_t, 
    Z_t, \bm{z}_t, \{ (\mu, \sigma^2, f) \} &\simindep 
    \begin{cases}
        \Ndist \left(\mu_0, \sigma_0^2 \right) & \text{if} \ Z_t = 0, \\
        \Ndist \left(\mu_{\bm{z}_t}^{(1)} + f_{\bm{z}_t}^{(1)}(x_{t,{\bm{z}_t}}), \sigma_{1,{\bm{z}_t}}^2 \right) & \text{if} \ Z_t = 1, \\
        \Ndist \left( \mu^{(Z_t)} + f^{(Z_t)} ( 
            \bm{x}_t(\bm{z}_t)
            %x_{t,(\bm{z_t})_1}, \ldots,  x_{t,(\bm{z_t})_r}
        ), \sigma_{Z_t}^2 \right) & \text{if} \ Z_t > 1,
    \end{cases} \nonumber \\
    & \qquad  \text{for} \ t = L+1, \ldots, T,  \\
    \Pr(Z_t = r \mid \bm{\Lambda}) &= \Lambda_r, \quad %\nonumber \\
\Pr(\bm{z}_t = (\ell_1, \ldots, \ell_r) \mid Z_t = r, \bm{\lambda}^{(r)}) = \lambda_{(\ell_1 , \ldots, \ell_r)}^{(r)}, \nonumber \\
    \text{for} \ r & = 0,1,\ldots,L, \ \text{independently for} \ t=L+1,\ldots,T, \nonumber \\
    \bm{\Lambda} &\sim \SBM( \eta_\Lambda, \pi_{\Lambda,1}, \pi_{\Lambda,3}, \bm{\gamma}_\Lambda, \bm{\delta}_\Lambda )\, , \nonumber  \\
    \bm{\lambda}^{(1)} \sim \SBM(\eta_\lambda, \pi_{\lambda,1}, \pi_{\lambda,3}, & \bm{\gamma}_\lambda, \bm{\delta}_\lambda),  \quad 
     \bm{\lambda}^{(r)} \simindep \SDM(\bm{\alpha}_{\lambda^{(r)}}, \beta_{\lambda^{(r)}}) \quad \text{for } r = 2, \ldots, R, \nonumber % \\
    % \mu_\ell \simindep \Ndist\left(m_0^{(\ell)}, v_0^{(\ell)}\right), \ \sigma_\ell^2 &\simindep \IGdist \left( \nu_\sigma^{(\ell)}/2, \nu_\sigma^{(\ell)}s_0^{(\ell)}/2 \right) \quad \text{for} \ \ell = 0,1,\ldots,L, \nonumber \\
    % f_\ell \mid \kappa_\ell, \sigma_\ell^2, \nu, \psi_\ell &\simindep \GP \left( \bm{0}, \kappa_\ell \sigma_\ell^2 \rho(x, x'; \nu, \psi_\ell) \right) \quad \text{for} \ \ell = 0,1,\ldots,L, \nonumber \\
    % \kappa_\ell \mid \nu_\kappa, \kappa_0 &\simindep \IGdist \left( \nu_\kappa/2, \nu_\kappa \kappa_0/2 \right) \quad \text{for} \ \ell = 0,1,\ldots,L, \nonumber \\ 
    % \psi_\ell \mid \nu_\psi, \psi_0 &\simindep \IGdist \left( \nu_\psi/2, \nu_\psi \psi_0/2 \right) \quad \text{for} \ \ell = 0,1,\ldots,L, \nonumber \\
    % p(\nu_\kappa) &\propto 1_{( \nu_\kappa \in \mathcal{V}_\kappa )}, \ \kappa_0 \sim \Gammadist(a_\kappa, b_\kappa), \nonumber \\
    % p(\nu_\psi) &\propto 1_{( \nu_\psi \in \mathcal{V}_\psi )}, \ \psi_0 \sim \Gammadist(a_\psi, b_\psi),
\end{align}
where $\bm{x}_t(\bm{z}_t)$ refers to the elements of $\bm{x}_t$ selected by $\bm{z}_t$; the top level implicitly conditions on lags in $\bm{x}_t$; %$\pi_k = (\pi_{k,0}, \ldots, \pi_{k,L-1})$ for $k=0,1$ allows for changing mixture weights in the SBM prior;
and the SDM prior density is proportional to the product of a Dirichlet density, having shape parameter vector $\bm{\alpha}_{\lambda^{(r)}}$, with $ \sum_{1 \le \ell_1 < \ldots < \ell_r \le L} ( \lambda_{(\ell_1, \ldots, \ell_r)}^{(r)} )^{\beta_{\lambda^{(r)}}} $ \citep{heiner2019spv}. The remaining hierarchical structure follows with (\ref{eq:hier}), except that $\psi^{(r)}$ for $r>1$ is replaced by a vector of parameters used to construct $\bm{\Psi}^{(r)}$ through, for example, some factorization that preserves positive definiteness.


% A simple modification to the GPMMTD model can yield selection of an optimal time delay in addition to dependence order. 
Most time-series analyses are conducted at the data-sampling time step without further consideration of sampling frequency, which can substantially affect inferences and forecasts. For example, sampling at high frequency %and analyzing relatively few lags 
can cause nonlinear dynamics to appear linear. Thus, in addition to dependence order, an optimal time delay is sometimes sought %in time-delay-embedding applications 
\citep[p.\ 38]{kantz2004}, and easily accommodated in the GPMMTD framework. %Joint inference for both is easily accommodated through a trivial adjustment to the GPMMTD framework. 
As before, the outer sum in (\ref{eq:GPMMTDtrans}) mixes over possible orders. However, instead of enumerating all lag combinations of order $r$ up to horizon $L$, the inner sum could index spacing among the $r$ lags so that component $\ell$ corresponds to the lag set $(\ell, 2\ell, \ldots, r\ell)$. For example, when $r=2$, the first component corresponds to lags $(1,2)$, the second component corresponds to lags $(2,4)$, the third to $(3,6)$, and so forth. This arrangement is less general in that it assumes relevance of all lags at the selected sampling frequency, up to the active order. Note also that estimation requires a longer time series, and that the model changes the dependence time step, but not the forecast time step. Nevertheless, this framework can substantially reduce the number of components under consideration and provide a parsimonious vehicle for modeling long-range dependence.



